ChildDiffusion: Unlocking the Potential of Generative AI and Controllable Augmentations for Child Facial Data using Stable Diffusion and Large Language Models

In this research work we have proposed high-level ChildDiffusion framework capable of generating photorealistic child facial samples and further embedding several intelligent augmentations on child facial data using short text prompts, detailed textual guidance from LLMs, and further image to image transformation using text guidance control conditioning thus providing an opportunity to curate fully synthetic large scale child datasets. The framework is validated by rendering high-quality child faces representing ethnicity data, micro expressions, face pose variations, eye blinking effects, facial accessories, different hair colours and styles, aging, multiple and different child gender subjects in a single frame. Addressing privacy concerns regarding child data acquisition requires a comprehensive approach that involves legal, ethical, and technological considerations. Keeping this in view this framework can be adapted to synthesise child facial data which can be effectively used for numerous downstream machine learning tasks. The proposed method circumvents common issues encountered in generative AI tools, such as temporal inconsistency and limited control over the rendered outputs. As an exemplary use case we have open-sourced child ethnicity data consisting of 2.5k child facial samples of five different classes which includes African, Asian, White, South Asian/ Indian, and Hispanic races by deploying the model in production inference phase. The rendered data undergoes rigorous qualitative as well as quantitative tests to cross validate its efficacy and further fine-tuning Yolo architecture for detecting and classifying child ethnicity as an exemplary downstream machine learning task.

==> Table/tab5.tex <==
\begin{table*}[!thpb]
\centering
\caption{Race detection results.}
\label{tab5}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\hline \hline
\multirow{2}{*}{} &
  \multicolumn{2}{c|}{African} &
  \multicolumn{2}{c|}{Asian} &
  \multicolumn{2}{c|}{White} &
  \multicolumn{2}{c|}{Hispanic} &
  \multicolumn{2}{c}{Indian} \\ \cline{2-11} 
 &
  \multicolumn{1}{c|}{Boy} &
  Girl &
  \multicolumn{1}{c|}{Boy} &
  Girl &
  \multicolumn{1}{c|}{Boy} &
  Girl &
  \multicolumn{1}{c|}{Boy} &
  Girl &
  \multicolumn{1}{c|}{Boy} &
  Girl \\ \hline
Deepface-Race &
  \multicolumn{1}{c|}{99.88\%} &
  99.63\% &
  \multicolumn{1}{c|}{96.24\%} &
  84.89\% &
  \multicolumn{1}{c|}{95.58\%} &
  84.20\% &
  \multicolumn{1}{c|}{97.56\%} &
  92.07\% &
  \multicolumn{1}{c|}{89.88\%} &
  87.95\% \\ \hline
Deepface-Gender &
  \multicolumn{1}{c|}{98.25\%} &
  57.74\% &
  \multicolumn{1}{c|}{80.85\%} &
  63.83\% &
  \multicolumn{1}{c|}{35.10\%} &
  93.53\% &
  \multicolumn{1}{c|}{91.94\%} &
  96.58\% &
  \multicolumn{1}{c|}{99\%} &
  84.94\% \\ \hline \hline
\end{tabular}
}
\end{table*}
